Orthogonal Random Forest for Causal Inference

We propose the orthogonal random forest, an algorithm that combines Neyman-orthogonality to reduce sensitivity with respect to estimation error of nuisance parameters with generalized random forests (Athey et al., 2017)--a flexible non-parametric method for statistical estimation of conditional moment models using random forests. We provide a consistency rate and establish asymptotic normality for our estimator. We show that under mild assumptions on the consistency rate of the nuisance estimator, we can achieve the same error rate as an oracle with a priori knowledge of these nuisance parameters. We show that when the nuisance functions have a locally sparse parametrization, then a local $\ell_1$-penalized regression achieves the required rate. We apply our method to estimate heterogeneous treatment effects from observational data with discrete treatments or continuous treatments, and we show that, unlike prior work, our method provably allows to control for a high-dimensional set of variables under standard sparsity conditions. We also provide a comprehensive empirical evaluation of our algorithm on both synthetic and real data.

==> comparison.tex <==
\section{Alternative ORF}


Recall that the nuisance functions $h$ are parameterized by
$x$-dependent vectors $\nu: \cX\rightarrow \reals^N$, i.e.
$h(x, W) = g(W; \nu(x))$ for some known functional form $g$. 

We consider a modification of the ORF algorithm. The algorithm takes
the input data set $D$ and randomly splits into two halves $D_1$ and
$D_2$, each with $n$ observations. The algorithm first builds a random
forest on the first data set $D_1$.  Then for every $Z_i\in D_2$, we
can use first random forest find a set of kernel weights $K(x_i, x_j)$
that measures the closenesss between $x_i$ and every observation $j$
in $D_1$.  Then for each point $Z_i\in D_2$, we will use the kernel
weights to compute a nuisance estimate $\hat \nu(x_i)$.  Furthermore,
we will find the nearest neighbor in $D_2$ to the target point $x$,
that is the observation $Z_i\in D_1$ such that
$i^* = \argmin_{Z_i \in D_2} \|x_i - x\|$. We will then use its
nuisance parameter $\hat\nu(x_{i^*})$ as the nuisance estimate
$\hat \nu$ for the target point.

Next we will use the second data set $D_2$ to build a second
forest. Given our target point $x$, we can assign forest-based weights
$a_{i}$ to each observation $Z_i\in D_2$, which measures the
similarity between the $x_i$ and $x$. Then our final target estimate $\hat \theta$ is computed as:
\[
  \hat \theta \quad \mbox{ solves: }\quad \sum_{i\in D_2} a_i
  \psi(Z_i; \hat \theta, g(W_i; \hat \nu)) = 0
\]

To establish our accuracy guarantee, we would require that the
nuisance function $\hat h$ given by the paramter $\hat \nu$ satisfies
\begin{equation}
    \E\bb{\|\hat{h}(W) - h(W)\|^2 | x} \leq \chi_{n,\delta}
\end{equation}
with probability $1 - \delta$.

Note that for any $W$, we can write
\begin{align*}
  \| \hat h(W) - h(W) \| &= \|g(W, \nu_0(x)) - g(W, \nu_0(x_{i^*})) +
  g(W, \nu_0(x_{i^*})) - g(W, \hat \nu_0(x_{i})) \| \\
&\leq \|g(W, \nu_0(x)) - g(W, \nu_0(x_{i^*}))\| + \|g(W, \nu_0(x_{i^*})) - g(W,
  \hat \nu_0(x_{i^*})) \|
\end{align*}
Given the Lipschitzness assumptions on $\nu_0$ and $g$, we can bound
the first term above as long as the distance $\|x - x_{i^*}\|$ is
bounded, and can bound the second term as long as the recovery error
is low $\|\nu_0(x_{i^*}) - \hat \nu_0(x_{i^*})\|$.

\begin{claim}
Suppose that for any fixed target point 
\end{claim}



\swcomment{We are agnostic about how the splitting works for now since
  the theory does not depend on it.}


\swcomment{However, the fact that $\hat h$ depends on the second
  dataset breaks the $U$-statistic definition?}



%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main.tex"
%%% End:


==> experimental.tex <==
% !TEX root=paper.tex
We show in Figure \ref{fig:example1} the quality of our estimates for
the PLR model.  The observations are generated according to the
Equations \eqref{maineq} and \eqref{confounding}. We perform
estimation using an orthogonal random forest with $20$ trees, where
each tree is computed on a random subsample with size $90\%$ of the
input data size.\footnote{We implement bootstrap subsampling (with
  replacement) even though subsampling without replacement is more
  convenient for proving our consistency result.} For $n=1000$, we
require a minimum leaf size of $50$ and at most $20$ splits, and for
$n=10000$, we require a minimum leaf size of $150$. The tree learner
only considers approximately balanced splits, that is, each child
should contain at least $30\%$ of the samples of the parent. Instead
of exactly solving kernel regression in Equation \eqref{ols}, we
perform a local estimate $\hat \theta_b$ in each tree and then take
average among these estimates. This is a computationally more
efficient since we need to evaluate our estimations for a large number
of target features. In Figure \ref{fig:example2}, we compare our
approach with a baseline approach where we residualize the variables
first using the whole sample to fit the first stage Lasso regressions
and then apply the generalized random forest of \cite{ATW17}. We see
that due to the non-linearity in $x$, the first stage Lasso estimates
are heavily biased since they are not fitted locally at the leafs and
this bias cannot be amended by the robustness of orthogonality. On the
contrary, running local Lasso regressions at the leafs leads to a much
smaller error.


\begin{figure}[htpb]
\centering
\subfigure[n=1000]{
\includegraphics[scale=.3]{plr_n_1000_p_500_s_30_dml_min_leaf_50.png}}
\subfigure[n=10000]{
\includegraphics[scale=.3]{plr_high_dim_orthogonal.png}}
\caption{$p=500$, $k=30$,  $d=1$ and $\theta(x)= 3 x^2 1\{x<.2\} + 3 (x^2 + 1) 1\{.2\leq x < .6\} + (6 x + 2) 1\{x\geq .6\}$.
The figures depict the mean and the $10\%$-$90\%$ interval of $50$ runs of the experiment.
}
\label{fig:example1}
\end{figure}

\begin{figure}[htpb]
\centering
\subfigure[orthogonal forest]{
\includegraphics[scale=.3]{plr_step_n_1000_res_at_leafs.png}}
\subfigure[a-priori residualization]{
\includegraphics[scale=.3]{plr_residualize_a_priori_n_1000.png}}
\caption{Comparison between orthogonal forest and the alternative of residualizing first and then running a generalized random forest on the residuals. $p=500$, $k=30$,  $d=1$ and $n=1000$.
The figures depict the mean and the $10\%$-$90\%$ interval of $50$ runs of the experiment.
}
\label{fig:example2}
\end{figure}

We also perform experiment with low-dimensional non-parametric
nuisance functions, where $f_0$ and $g_0$ are only functions of a
single dimensional confounder/control $X$. We generated data where
$f_0$ and $g_0$ where high-degree polynomials (in particular
$f_0(X)=.2X + .4X^2 + X^4$ and $g_0(X) = X + X^2 + .2 X^3 + .5x^6$ and
) and perform a third-degree polynomial regression to fit each of
these functions. In the case of single-dimension, we can actually very
nicely visualize the random forest fitted by our approach and we see
that it picks up the exact points of discontinuity of the treatment
effect quite acurately.

\begin{figure*}[htpb]
\centering
\subfigure[Example Constructed Tree]{
\includegraphics[scale=.1]{monte_tree.png}}
\subfigure[Local Two-Stage Estimation]{
\includegraphics[scale=.3]{nn_Tree0_lll.png}}
\subfigure[Fitted Effect $n=2000$]{
\includegraphics[scale=.3]{poly_fit_n_2000.png}}
\caption{Example tree and local orthogonal regression run at the leaf. The fitted effect on the right was produced by running $50$ experiments, each containing $n=2000$ samples. The figures depict the mean and the $10\%$-$90\%$ interval of $50$ runs of the experiment.
}
\label{fig:example2}
\end{figure*}

==> lasso.tex <==
% !TEX root = nips_2018.tex
\section{Nuisance Estimation with Kernel Lasso}\label{sec:kernel-lasso}
We now study the error rate of Lasso as our nuisance estimation
method. Recall that the nuisance estimate $\hat h$ is the
parameterized by two vectors $\hat \gamma$ and $\hat q$, which are
obtained by solving two Lasso regression problems in
\Cref{lasso1,lasso2}.
% \vscomment{Shouldn't this be $\gamma$ and not $\gamma(x)$
% below. Also shoulnd't it be $q_b(x)$ above?}
% \begin{align}
%   \hat \gamma_b &= \argmin_{\gamma} \frac{1}{2|H_b|} \sum_{Z_i\in H_b} (T_i
%                   -\langle W_i, \gamma)^2 + \lambda_\gamma \|\gamma\|_1\\
%   \hat q_b &= \argmin_{q} \frac{1}{2|H_b|} \sum_{Z_i\in H_b} (Y_i - \langle W_i, q\rangle)^2 + \lambda_q \|q\|_1
% \end{align}
% where $\lambda_\gamma$ and $\lambda_q$ are appropriately chosen
% regularization parameters. 
Then the error of the nuisance estimate $\hat h$ can be written as
\[
  \|\hat h(W) - h_0(W)\|_2^2 = (\langle \hat q - q_0(x), W\rangle)^2 +
  (\langle \hat \gamma - \gamma_0, W\rangle)^2
\]
where $q_0(x) = \theta_0(x)\gamma_0 + \beta_0$ for any $x$. Thus,
it suffices to bound the $\ell_2$ error of the sparse vectors:
$\|\hat q - q_0(x)\|_1$ and $\|\hat \gamma - \gamma_0\|_1$. 
 \iffalse
We will rely on the following assumptions on the partial linear
regression (PLR) model.



\begin{assumpt}\label{plrass}

The PLR model satisfies the following:
\iffalse
\item The functions $\gamma_0, \beta_0\colon \RR^d \rightarrow \RR^p$
  are 1-Lipschitz in the sense that for any $x', x''\in \RR^d$,
  \begin{align*}
  \|\beta_0(x') - \beta(x'')\|_1, \|\gamma_0(x') - \gamma(x'')\|_1 \leq \|x' - x''\|_2% \; &\leq \|x' - x''\|_2
  \end{align*}
  and $\theta_0\colon \RR^d \rightarrow \RR$ is 1-Lipschitz.  
% \item The function $\theta$ is L-Lipschitz in the feature vector $x$
%   for some constant $L$.
\item For any feature vector $x'$, $\|\gamma_0(x)\|_1 \leq O(1)$.
\fi
\begin{enumerate}
\item $\theta_0\colon \RR^d \rightarrow \RR$ is 1-Lipschitz, and
  $|\theta_0(x')|\leq 1$ for all $x'\in [0, 1]^d$.

\item The sparse vectors $\|\beta_0\|_1, \|\gamma_0\|_1 \leq O(k)$.


\item $\Ex{}{\eta^2 \mid x} \geq O(1)$.\swcomment{so that the
    derivative is invertible}


\item The control $W_i$ lies in the range of $[-1, 1]^p$, and for any
  feature $x_i$, the conditional covariance matrix satisfies
  \[
    \Ex{}{W_i W_i^\intercal \mid x_i} \succeq \lambda_0 I_p
  \]
  where $\lambda_0$ satisfies $1/\lambda_0 \leq O(1)$. The noise
  $\eta_i$ is has mean 0 conditioned on any values of $W_i, x_i, T_i$,
  $\eps_i$ has mean 0 conditioned on any values of $W_i, x_i$. We
  assume $|\eta_i|, |\eps_i| \leq 1$.
\iffalse
  \vscomment{I think we should replace this assumption with the
    following: For all $x$: i) the conditional expected covariance
    matrix $\Ex{}{W_i W_i^T | x_i}\succeq \alpha I_p$, ii) the
    distribution of the product of any two coordinates
    $\Sigma_{ijk} = W_{ij} X_{ik}$ conditional on $x$ is
    $\sigma$-subgaussian.}\sw{DONE}
\fi
\end{enumerate}
\end{assumpt}

The first two assumptions are standard Lipchitzness and boundedness
assumptions, while the last assumption is crucial for bounding the
Lasso error when the response noise is adversarially chosen.
\fi
Recall that for any observation $Z_i = (T_i, Y_i , W_i, x_i)$ in
the input data set, we have the following:
\begin{align}
  Y_i&= \langle W_i, q_0(x_i) \rangle + \eta_i \, \theta_0(x_i) + \eps_i \label{hey}\\
  T_i&= \langle W_i, \gamma_0 \rangle + \eta_i\label{man}
\end{align}
For each observation $i$, let $w_i = \sum_{b=1}^B w_{ib}$. To view our
weighted Lasso problem as a standard Lasso problem, we will consider
the following rescaled observation $(\tilde W_i, \tilde Y_i)$ such
that
\[
  \tilde W_i = \sqrt{w_i} W_i, \quad \tilde Y_i = \sqrt{w_i} Y_i,
  \quad \mbox{ and, } \quad \tilde T_i = \sqrt{w_i} T_i
\]
Then our Lasso estimates $\hat \gamma$ and $\hat q$ can be viewed as a
solution to
\begin{align}
  \hat \gamma =   \argmin_{\gamma} \frac{1}{2}\sum_{i} \left(\langle \tilde W_i, \gamma\rangle - \tilde
  Y_i \right)^2 + \lambda_\gamma \|\gamma\|_1\\
  \hat q =  \argmin_{q} \frac{1}{2}\sum_{i} \left(\langle \tilde W_i, q\rangle - \tilde
  Y_i \right)^2 + \lambda_q \|q\|_1.
\end{align}


Furthermore, to relate each observation $i$ to the target feature $x$,
we have the following relationship:
\begin{align*}
  \tilde T_i = \langle \tilde W_i, \gamma_0(x)\rangle + \underbrace{\sqrt{w_i} \eta_i}_{\tilde \cE_{i}^T},\quad \mbox{and,} \quad
  \tilde Y_i = \langle \tilde W_i, q_0(x)\rangle +\underbrace{\sqrt{w_i}{ \left( \Delta q(x, x_i, W_i) + \eta_i \theta_0(x_i) + \eps_i\right)} }_{\tilde\cE_{i}^Y}
\end{align*}
% \vscomment{I changed the underbrace to not include $\sqrt{w_i}$. I think that's how you use it in derivations below.}
where $\Delta q(x, x', X) = \langle X, (q_0(x') - q_0(x)) \rangle$.
Now we can view $\tilde Y_i$ and $\tilde T_i$ outcomes as generated
from a linear model with weight vectors $q_0(x)$ and $\gamma_0$ and
noise terms $\tilde\cE_i^Y$ and $\tilde\cE_i^T$. Then we can bound the
error of both $\hat q$ and $\hat \gamma$ by using the following result
on Lasso.

\begin{theorem}[Follows from Theorem 11.1 of
  \cite{Lasso-Book}]\label{lasso-err}
  Let $r_0\in \RR^p$ be a $k$-sparse vector and let $S$ be its
  support.  Consider a set of $n$ observations such that each
  observation $(\tilde W_i, \tilde Y_i)$ satisfies
  \[
    \tilde Y_i = \langle \tilde W_i , r_0 \rangle + \tilde\cE_i.
  \]
  Let $\bX\in \RR^{n\times p}$ denote the design matrix consisting the
  vectors $\tilde W_i$ as rows. Suppose $\bX$ satisfies the
  \emph{restricted eigenvalue (RE)} condition for $r_0$ with
  parameters $(3, \rho)$ that is
\[
  \frac{\nu \bX^\intercal \bX \nu}{\|\nu\|_2^2} \geq
  \rho \mbox{ for all non-zero } \nu\in C(S; 3)
\]
where
$C(S; 3) = \{\nu\in \RR^p \mid \|\nu_{S^c}\|_1 \leq 3 \|\nu_S\|_1\}$.
Then any estimate $\hat r$ obtained by solving
\[
  \hat r = \argmin_{r} \frac{1}{2}\sum_{i} \left( \langle \tilde W_i,
    r\rangle - \tilde Y_i \right)^2 + \lambda \|r\|_1
\]
satisfies the following error bound
\[
  \|\hat r - r_0\|_1 \leq O\left(\frac{1}{\rho} k
    \|\bX^\intercal \tilde\cE\|_\infty\right)
\]
as long as $\lambda \geq 2\|\bX^\intercal \tilde \cE\|_\infty$.
\end{theorem}


To invoke this result, we need two ingredients:
\begin{enumerate}
\item First, we will establish the restricted eigenvalue condition of
  $\bX$, where $\bX$ is the design matrix such that each row of $\bX$
  is the re-scaled vector $\tilde W_i$.
\item Then we will also provide bounds on
  $\|\bX^\intercal \tilde\cE^Y\|_\infty$ and
  $\|\bX^\intercal \tilde\cE^T\|_\infty$. The analysis for bounding
  the $\ell_2$ error of $\hat q_b$ is more challenging since the noise
  terms $\cE_i^Y$ does not have mean 0.
\end{enumerate}






\iffalse
Let us first recall the definition of restricted eigenvalue.
\begin{definition}[Restricted Eigenvalue Condition]
  The matrix $\bX$ satisfies the \emph{restricted eigenvalue (RE)}
  condition with parameters $(\tau, \rho)$ if
\[
  \frac{\nu \bX^\intercal \bX \nu}{\|\nu\|_2^2} \geq
  \rho \mbox{ for all non-zero } \nu\in C(S; \tau)
\]
where
$C(S; \tau) = \{\nu\in \RR^p \mid \|\nu_{S^c}\|_1 \leq \tau
\|\nu_S\|_1\}$ and $S$ is the support of
$q_0(x) = \theta_0(x) \gamma_0 + \beta_0$.
\end{definition}
\fi


\iffull
\subsection{Restricted Eigenvalue Condition for $\bX$}
% Let $S$ be a subset of the input data set $\{Z_1, \ldots,
% Z_n\}$. Then given any permutation over $S$, we also can define a
% equal partition $S^1, S^2, S^3$ of the set $S$. \swcomment{assuming
% $s$ is divisible by 3} Then let $\Sigma(S, \pi)$ denote the matrix
% $\sum_{i=1}^n w_{ib} X_{i} X_{i}^\intercal$, with weights obtained
% by running the tree learner on $S$ with partition
% $S^1, S^2, S^3$.\swcomment{This is a bit mouthful for now}

For any set of observations $S\subset D_1$ of size $s$, let $\pa(J)$
denotes the set of all possible equal partitions $(S^1, S^2)$ of $S$
such that the cardinalities of the two subsets differ by at most
1. Then let $\Sigma(S^1, S^2)$ denote the matrix
$\sum_{Z_i \in J} K(x_i, x, (S^1, S^2)) X_{i} X_{i}^\intercal$, with
weights $K(x_i, x, (S^1, S^2))$ obtained by running the tree learner
on $S$ with partition $(S^1, S^2)$. Consider the following matrix
\[
  \hat \Sigma(D_1) = \frac{1}{{n \choose s}} \sum_{S\subset D_1: |S| =
    s} \frac{1}{|\pa(S)|}\sum_{(S^1, S^2)\in \pa(S)} \Sigma(S^1, S^2)
\] 
Observe that each entry of the matrix $\hat \Sigma(D_1)$ is a
U-statistic. Let $\Sigma=\Ex{}{\hat \Sigma^U(D_1)}$. The following
lemma bounds the minimum eigenvalue of $\Sigma$.

% follows from the fact that the conditional expected covariance
% matrix
% $\Sigma = \Ex{}{\tilde W_i \tilde W_i^\intercal \mid x_i} \succeq
% \lambda_0I_p$.

\begin{lemma}
  Under \Cref{plrass}, taking over the random draws of $D_1$, the
  expectation satisfies
  $$\Sigma \succeq \lambda_0 I_p.$$
\end{lemma}

\begin{proof}
  By linearity of expectation, it suffices to show that for any random
  subset $S$ and any random equal partition $(S^1, S^2)$,
  \[
    \Ex{}{\Sigma(S^1, S^2)} \succeq \lambda_0 I_p.
  \]
  Since only observations in $S^2$ have non-zero weights, we have
  \[
    \Sigma(S^1 , S^2) = \sum_{Z_i\in S} K(x_i, x, (S^1, S^2)) W_i W_i^\intercal =
    \sum_{Z_i\in S^2} K(x_i, x, (S^1, S^2)) W_i W_i^\intercal
  \]
  Note that for each observation $Z_i$ in $S^2$, the weight $K(x_i, x, (S^1, S^2))$ is
  only a function of $S^1$ and the feature $x_i$. By honesty, we have
  for each $Z_i \in S^2$,
  \begin{align*}
    \Ex{}{ K(x_i, x, (S^1, S^2)) W_i W_i^\intercal} &= \Ex{x_i, S_1}{ \Ex{}{K(x_i, x, (S^1, S^2)) W_i
                                                      W_i^\intercal\mid x_i, S_1}}\\ &= \Ex{x_i, S_1}{\Ex{}{K(x_i, x, (S^1, S^2)) \mid
                                                                                       x_i, S_1}\Ex{}{W_i W_i^\intercal \mid x_i,
                                                                                       S_1}}\\ 
                                                    &\succeq \Ex{}{K(x_i, x, (S^1, S^2)) \lambda_0 I_p}
  \end{align*}
  Then the stated bound follows directly from the fact the weights are
  non-negative and sum to 1.
\end{proof}


We can also derive a concentration inequality for each entry of the
matrix $\hat \Sigma(D_1)$ by relying on the standard concentration result
on U-statistic.


\begin{theorem}
  For any $\eps > 0$ and any pair $(l, j)\in [p]^2$,
  \[
    \Pr_{Z_1, \ldots, Z_n}\left[ \left|\hat \Sigma(D_1)_{lj} -
        \Sigma_{lj}\right| \geq \eps \right] \leq 2\exp\left( -
      \frac{(n/s)\eps^2}{2}\right)
  \]
  Equivalently, for any $\delta \in (0, 1)$, with probability
  $1 - \delta$,
  $\left|\hat \Sigma(D_1)_{lj} - \Sigma_{lj}\right| \leq
  \sqrt{\frac{2}{n/s} \ln(2/\delta)}$.
\end{theorem}

By taking a union bound over all pairs $(l, j)\in [p]^2$, we can show
that with probability at least $1 - \delta$, 
\[
  \left \| \hat \Sigma(D_1) - \Sigma \right\|_\infty \leq
  \sqrt{\frac{4s}{n}\ln(p/\delta)}.
\]

Now we can rewrite the covariance matrix as
\[
  \bX^\intercal\bX = \sum_{Z_i \in D_1} \tilde W_i \tilde
  W_i^\intercal = \sum_{Z_i \in D_1} w_i W_i W_i^\intercal =
  \frac{1}{B} \sum_{Z_i\in D_1} \sum_{b=1}^B K(x_i, x , (S_b^1,
  S_b^2))\left( W_i W_i^\intercal\right)
\]
Since the subsets $S_b$ and the partitions $(S_b^1, S_b^2)$ are
randomly selected, we can view $\bX^\intercal \bX$ as a Monte Carlo
approximation of $\hat \Sigma(D_1)$. Furthermore, by standard Chernoff
bound, we know that as long as the number of trees is bigger than
$n/s$, the error introduced by the Monte Carlo approximation will be
subsumed by the U-statistic error.

\begin{corollary}\label{linfty}
  As long as the number of trees $B \geq \left(n/s\right)$, the
  following inequality holds with probability at least $1 - \delta$, 
  \[
    \left\| \bX^\intercal \bX - \Sigma \right\|_\infty \leq
    O\left(\sqrt{\frac{s}{n} \ln(p/\delta)}\right).
  \]
\end{corollary}



\begin{lemma}\label{rho-bound}
  Suppose that the number of trees $B\geq n/s$. Let $r$ be a sparse
  vector in $\RR^p$ with a support size at most $O(k)$. With
  probability at least $1 - \delta$, the matrix $\bX$ satisfies the
  restricted eigenvalue condition for $r$ with parameters $(3, \rho)$,
  where
  \[
    \rho \geq \lambda_0 - O\left(k \sqrt{\frac{s}{n}\ln(p/\delta)}
    \right)
  \]
\end{lemma}

\begin{proof}
  Let $r$ be a $k$-sparse vector in $\RR^p$ and let $S(r)$ be the
  support of $r$. Let $\nu \in C(S(r); 3)$. To simplify notation, let
  $M = \bX^\intercal \bX - \Sigma$. Then we can write
  \begin{align*}
    \tag{Cauchy-Swartz}    \frac{\nu^\intercal M \nu}{\|\nu\|_2^2} &\leq     \frac{\|\nu\|_1\| M \nu\|_\infty}{\|\nu\|_2^2}\\
    \tag{Cauchy-Swartz}                                           &\leq    \frac{\|\nu\|_1\| M\|_\infty \|\nu\|_1}{\|\nu\|_2^2}\\
                                                                  &\leq    \frac{\|\nu\|_1^2\| M\|_\infty}{\|\nu\|_2^2}\\
  \end{align*}
  Let $S^c$ denote the complement of $S(r)$, and let $\nu_S$ and
  $\nu_{S^c}$ denote the subvectors of $\nu$ over the coordinates in
  $S^c$.  By the definition of $C(S(r), 3)$, we know that
  \[
    \|\nu\|_1 = \|\nu_S\|_1 + \|\nu_{S^c}\|_1 \leq 4 \|\nu_S\|_1
  \]
  It follows that
  \begin{align*}
    \frac{\|\nu\|_1^2}{\|\nu\|_2^2} \leq \frac{\left(4\|\nu_{S}\|_1\right)^2}{\|\nu\|_2^2} \leq 16 \frac{\|\nu_S\|_1^2}{\|\nu_S\|_2^2} = 16 |S|
  \end{align*}
  Note that $|S| = O(k)$. By \Cref{linfty}, we have with probability
  at least $1 - \delta$ that
  $\|M\|_\infty\leq O\left(\sqrt{\frac{s}{n}\ln(p/\delta)} \right)$,
  and so
  \[
    \frac{\nu^\intercal M \nu}{\|\nu\|_2^2} \leq 16  \|M\|_\infty |S| \leq O\left(k\sqrt{\frac{s}{n}\ln(p/\delta)}  \right)
  \]
  which completes the proof.
\end{proof}


\subsection{Bounding the Noise Terms}
Next, we show that both $\|\bX^\intercal \tilde\cE^Y\|_\infty$ and
$\|\bX^\intercal \tilde \cE^T\|_\infty$ are bounded with high
probability. First, note that for each $j\in [p]$,
\begin{align*}
  \langle \bX^j , \tilde \cE^Y \rangle &= \sum_i
  w_i W_{ij} \left( \langle W_i, q_0(x_i) - q_0(x)\rangle + \eta_i
  \theta_0(x_i) + \eps_i\right)\\
  \langle \bX^j , \tilde \cE^T \rangle &= \sum_i
  w_i W_{ij} \eta_i
% \leq \left(\max_{i\colon w_i \neq 0}
    % |\cE^Y_i|\right) \left|\sum_i w_i W_{ij}\right|
\end{align*}
\iffalse we will bound the magnitude of each coordinate of $\cE^Y$.
\begin{lemma}\label{cebound}
  Under \Cref{plrass}, for any $\delta \in (0, 1)$, with probability
  at least $1 - \delta$, the following bounds hold for all
  $i \in [n]$:
  \begin{align*}
    |\cE_i^Y|
    &\leq
      O\left( \|x - x_i\|_2 \|\gamma_0\|_1 + \sqrt{\log(n/\delta)} \right)
\end{align*}
\end{lemma}
\fi It suffices to bound $\max_j \langle \bX^j , \tilde \cE^Y \rangle$
and $\max_j \langle \bX^j , \tilde \cE^T \rangle$. We will first
define several useful functions. First, for any $j\in [p]$, any subset
$S$ of $D_1$ of size $s$, along with any equal partition $(S^1, S^2)$,
define
\begin{align*}
  R_j^Y(S^1, S^2) &= \sum_{Z_i\in S} K(x_i, x, (S^1, S^2)) \, W_{ij}
                    \left(\Delta q(x, x_i, W_i) + \eta_i \theta_0(x_i) + \eps_i\right)\\
  R_j^T(S^1, S^2) &= \sum_{Z_i\in S} K(x_i, x, (S^1, S^2))\, W_{ij}\eta_i
\end{align*}
with weights $K(x_i, x, (S^1, S^2))$ obtained by running the tree
learner with the partition $(S^1, S^2)$. Now consider the following
two U-statistics for each $j\in [p]$,
\begin{align*}
  \hat R_j^Y(D_1) &= \frac{1}{{n \choose s}} \sum_{S\subset D_1: |S|= s} \frac{1}{s!} \sum_{(S^1, S^2)\in \pa(S)} R_j^Y(S^1, S^2)\\
  \hat R_j^T(D_1) &= \frac{1}{{n \choose s}} \sum_{S\subset D_1: |S|= s} \frac{1}{s!} \sum_{(S^1, S^2)\in \pa(S)}
                    R_j^T(S^1, S^2)
\end{align*}


The following bound on $\Delta q(x, x', X)$ will be a useful tool.

\begin{lemma}\label{ohboy}
  For any $x, x', W$,
  $\|\Delta q(x, x', W) \|_1 \leq \|x - x'\|_2 \|\gamma_0\|_1$.
\end{lemma}

\begin{proof}
We can write:
\begin{align*}
  \|\Delta q(x, x', W)\|_1  &\leq { \left( \|W\|_\infty \| q_0(x')
                              - q_0(x)\|_1\right)} \tag{Cauchy-Swartz}\\
                            &\leq {  \| q_0(x')
                              - q_0(x)\|_1}\tag{boundedness of $X$}\\
                            &=  \| \theta_0(x')\gamma_0 - \theta_0(x)\gamma_0\|_1\\
                            &= \|\gamma_0\|_1 |\theta_0(x') - \theta_0(x)|\\
                            &\leq \|\gamma_0\|_1 \|x' - x\|_2\tag{Lipschitzness of $\theta_0$}
\end{align*}
which completes the proof.
\end{proof}



\iffalse Since each $W_{ij}$ is drawn independently from the uniform
distribution over $[-1, 1]$ conditioned on any realization of the the
weights $w_{ib}$, we have
$\Ex{Z_1,\ldots , Z_n}{R_j^U} = 0$.\swcomment{may want to add a proof
  for this} The following result follows from the standard
concentration inequality of U-statistic.  \fi

The following lemma bounds the expected value of the U-statistic. In
particular, we can bound the expectation of $\hat R^Y_j(D_1)$ using
the shrinkage of the leaf size in the tree.


\begin{lemma}
  Taking expectation over the random draws of $D_1$, the following
  holds for each $j\in[p]$,
  \[ 
    \Ex{}{\hat R_j^T(D_1)} = 0 ,\qquad \mbox{ and, } \qquad\Ex{}{\hat
      R_j^Y(D_1)} \leq O\left( k \right) \, \Ex{D_1, S^1,
      S^2}{\max_{i\in D_1} \|x - x_i\|_2 \mid K(x_i , x, (S^1, S^2)) >
      0}.
  \]
\end{lemma}


\begin{proof}
  By linearity of expectation, we have
  $\Ex{}{\hat R_j^T(D_1)} = \Ex{}{R_j^T(S^1, S^2)}$ and
  $\Ex{}{\hat R_j^Y(D_1)} = \Ex{}{R_j^Y(S^1,S^2)}$, where the
  expectations of the right hand sides are taken over the random draws
  of $D_1$, random subset $S$ and random equal partition $(S^1,
  S^2)$. The expectation of $R_j^T(S^1, S^2)$ is
  \[
    \Ex{}{R_j^T(S^1, S^2)} = \Ex{}{\sum_{Z_i \in S} w_{i}
      W_{ij}\eta_i} = \Ex{}{\sum_{Z_i\in S^2} K(x_i, x, (S^1, S^2))\, W_{ij} \eta_i}
  \]
  where the second equality follows since $K(x_i, x, (S^1, S^2))\,$ is non-zero only for
  $Z_i\in S^2$.  Similarly,
\begin{align*}
  \Ex{}{  R_j^Y(S^1, S^2) }  &= \Ex{}{\sum_{Z_i\in S^2} K(x_i, x, (S^1, S^2))W_{ij} \left(\Delta
                               q(x, x_i, W_i) + \eta_i \theta_0(x_i) + \eps_i
                               \right)}\\
                             & = \Ex{}{\sum_{Z_i\in S^2} K(x_i, x, (S^1, S^2))W_{ij} \left(\Delta
                               q(x, x_i, W_i)
                               \right)} + \Ex{}{\sum_{Z_i\in S^2} w_{i}W_{ij} \left(\eta_i \theta_0(x_i) + \eps_i
                               \right) }
  \end{align*}
  First, recall that by our assumption of the PLR model, we have
  \begin{align}
    \Ex{}{\eps_i \mid W_i, x_i, T_i} = 0, \quad\Ex{}{\eta_i \mid x_i,
      W_i} = 0\label{mean0}
  \end{align}
  Note that the learner assigns the weight $w_{i}$ only depends on the
  subsample $S^1$ and the feature $x_i$. Therefore, by honesty of the
  weights and the law of iterated expectations, for each
  $Z_i \in S^2$,
  \begin{align}
    \Ex{}{K(x_i, x, (S^1, S^2))\, W_{ij}\eta_i} &= \Ex{x_i, W_i, S^1}{\Ex{}{K(x_i, x, (S^1, S^2))\, W_{ij}
    \eta_i\mid x_i, W_i}} \\ &= \Ex{x_i, W_i, S^1}{\Ex{}{K(x_i, x, (S^1, S^2))\, \mid x_i,
    W_i, S^1}\Ex{}{\eta_i W_{ij}\mid x_i, W_i, S^1}} = 0\label{malaka}
  \end{align}
  where the last equality follows from
  $\Ex{}{\eta_i W_{ij}\mid x_i, W_i, S^1} = \Ex{}{\eta_i\mid x_i, W_i,
    S^1}\Ex{}{ W_{ij}\mid x_i, W_i, S^1} = 0$, which implies that
  $\Ex{}{\hat R^T_j(D_1)} = 0$ by linearity of expectation.
  Similarly,
  \begin{align*}
&\;\;\;\;~~~~    \Ex{}{K(x_i, x, (S^1, S^2))\, W_{ij} (\eta_i \theta_0(x_i) + \eps_i)}\\ &= \Ex{W_i,
      x_i, S^1}{\Ex{}{ K(x_i, x, (S^1, S^2))\, W_{ij} (\eta_i \theta_0(x_i) + \eps_i)
        \mid W_i, x_i, S^1} }\\
 &= \Ex{W_i, x_i, S^1}{\Ex{}{ K(x_i, x, (S^1, S^2))\, \theta_0(x_i) W_{ij} \eta_i
        \mid W_i, x_i, S^1} } + \Ex{W_i, x_i, S^1}{\Ex{}{ K(x_i, x, (S^1, S^2))\, W_{ij} \eps_i
        \mid W_i, x_i, S^1} }
  \end{align*}
  By the same reasoning in \Cref{malaka}, the second term
  $\Ex{W_i, x_i, S^1}{\Ex{}{ K(x_i, x, (S^1, S^2))\, W_{ij} \eps_i \mid W_i, x_i, S^1} }
  = 0$. For the first term, we can write
  \begin{align*}
    & \Ex{W_i, x_i, S^1}{\Ex{}{ K(x_i, x, (S^1, S^2))\, \theta_0(x_i) W_{ij} \eta_i \mid
      W_i, x_i, S^1} }\\ = &\Ex{W_i, x_i, S^1}{\Ex{}{ K(x_i, x, (S^1, S^2))\,
                             \theta_0(x_i) W_{ij} \mid W_i, x_i, S^1} \Ex{}{ \eta_i \mid
                             W_i, x_i, S^1} } = 0
  \end{align*}
  Moreover, by \Cref{ohboy},
\begin{align*}
  \Ex{}{\sum_{Z_i\in S} K(x_i, x, (S^1, S^2))W_{ij} \left(\Delta
  q(x, x_i, W_i)
  \right)}\leq \Ex{}{\sum_{Z_i\in S} K(x_i, x, (S^1, S^2)) \left(  \|x_i - x\|_2 \|\gamma_0\|_1\right)}
  \end{align*}
  Then our claim follows directly from the fact that the sum of the
  weights equals 1 and that $\|\gamma_0\|_1\leq O(k)$.
\end{proof}


We can apply the standard concentration inequality for U-statistic
again.

\begin{theorem}
For any $\eps > 0$ and any $j\in [p]$, 
\[
  \Pr_{D_1} \left[\max\left\{\left|\hat R_j^T(D_1) - \Ex{}{\hat
          R_j^T(D_1)}\right| , \left| \hat R_j^Y(D_1) - \Ex{}{\hat
          R_j^Y(D_1)}\right|\right\} \geq \eps \right] \leq
  4\exp\left(- \frac{(n/s)\eps^2}{18} \right)
\]
Equivalently, for any $\delta\in (0, 1)$, with probability
$1 - \delta$, 
\[
  \max\left\{\left|\hat R_j^T(D_1) - \Ex{}{\hat R_j^T(D_1)}\right| ,
    \left| \hat R_j^Y(D_1) - \Ex{}{\hat R_j^Y(D_1)}\right| \right\}
  \leq \sqrt{\frac{18 s}{n} \ln(4/\delta)}.
\]
\end{theorem}


Now we can view
$\langle \bX^j , \tilde\cE^Y \rangle =
\frac{1}{B}\sum_{b=1}^B\sum_{i=1}^n w_{ib}W_{ij} \left(\Delta q(x,
  x_i, W_i) + \eta_i \theta_0(x_i) + \eps_i\right)$ as a Monte Carlo
approximation to the U-statistic $\hat R^Y_j(D_1)$, and view
$\langle \bX^j , \tilde\cE^T \rangle =
\frac{1}{B}\sum_{b=1}^B\sum_{i=1}^n w_{ib}W_{ij} \eta_i$ as a Monte
Carlo approximation to the U-statistic $\hat R^T_j(D_1)$. By Chernoff
bound, we know that as long as $B\geq n/s$ is sufficiently large, we
know that Monte Carlo approximation error will be subsumed by the
U-statistic deviation error.



\begin{corollary}\label{rjbound}
  As long as the number of trees $B\geq (n/s)$, with probability at
  least $1-\delta$, the following inequality holds 
  \begin{align*}
    & \max_j \left|\langle \bX^j , \cE^T \rangle\right| \leq       O\left(\sqrt{\frac{s}{n}\ln(p/\delta)}\right)\\
    & \max_j \left|\langle \bX^j , \cE^Y \rangle\right| \leq
      O\left(\sqrt{\frac{s}{n}\ln(p/\delta)} + k\, \Ex{D_1, S^1,
      S^2}{\max_{i\in D_1} \|x - x_i\|_2 \mid K(x_i, x, (S^1, S^2))
      > 0}\right)
  \end{align*}
\end{corollary}
\noindent Taking the kernel shrinkage result we establish in
\Cref{kernel-bound}, we obtain the following bound on
$\|\bX^\intercal \cE^Y\|_\infty$.



\iffalse
\begin{proof}
  Let $\bX^j$ denote the $j$-th column of the matrix $\bX$. Then our
  goal is to bound $\max_j |\langle \bX^j , \cE^Y \rangle|$. Moreover,
  for each $j$,
\[
  |\langle \bX^j , \cE^Y \rangle | = \left|\sum_i w_i \cE_i^Y
    W_{ij}\right| \leq \left(\max_{i\colon w_i \neq 0} |\cE^Y_i|\right) \left|\sum_i w_i W_{ij}\right|
\]

\vscomment{The final inequality above is wrong. Cauchy Scwarz requires $\sum_{i} |w_i W_{ij}|$ for the second term, which then does not concentrate well. Instead one needs to argue about the distribution of the random variable $V_{ij} = w_i \cE_i^Y W_{ij}$. This random variable is not mean zero, since if you expand it, it is of the form:
\begin{align*}
V_{ij} =~& X_j w_i\left( \Delta q(x, x_i, X) + \eta_i \theta_0(x_i) + \eps_i\right)\\
 =~&  X_j w_i\left( \langle X, (q_0(x') - q_0(x)) \rangle + \eta_i \theta_0(x_i) + \eps_i\right) 
\end{align*}
So its expected value is equal (assuming $\eta_i$ and $\epsilon_i$ are independent of $X$):
\begin{align*}
\Ex{}{V_{ij}}
 =~&  \Ex{}{X_j^2 w_i (q_{0j}(x') - q_{0j}(x))}\\
 \leq~& \Ex{}{X_j^2 w_i \|x'-x\|}
\end{align*}
However, by Kernel shrinkage the latter is upper bounded by $w_i s^{-\tau}\Ex{}{X_j^2}=O(w_i s^{-\tau})$. Since $\sum_{i} w_i = 1$ the mean of the random variable $\sum_i V_ij$ is upper bounded by $O(s^{-\tau})$. Subsequently if we also assume that the whole random variable $V_{ij}$ is sub-gaussian, then we get a concentration inequality around this mean by $U$-statistics of $\sqrt{\frac{s \log(1/\delta)}{n}}$.  This would hold if random variables are bounded or if $X_j$ is bounded and $\eta_i, \epsilon_i$ are sub-gaussian or the other way around. 
If $X_j$ are bounded in $[0, 1]$ then we can also analyze the above in an alternative manner: we first split the first component and bound it conditional on $X$ from kernel shrinkage
\begin{align*}
X_j w_i\left( \langle X, (q_0(x') - q_0(x)) \rangle \leq w_i \|x'-x\| \leq w_i s^{-\tau}\right)
\end{align*}
Then we analyze the second component:
\begin{align*}
X_j w_i\left( \eta_i \theta_0(x_i) + \eps_i\right) 
\end{align*}
This is bounded as long as the quantities $\left|\sum_{i} w_i W_{ij} \eta_i\right|$ and $\left|\sum_{i} w_i W_{ij} \eps_i\right|$ are bounded. These are quantities of the same form as in a normal lasso proof. So both fixed-design Gaussian errors and fixed-errors Gaussian design settings will work. In any case we should be getting a bound of the form: $O\left(s^{-\tau} + \sqrt{\frac{s\log(p/\delta)}{n}}\right)$, which is great. Appropriately tuning $s$ would give a good bound that would allow us to claim \emph{no effect} of the nuisance function estimation on the leading term of the MSE of the treatment effect estimate.
}

Then by \Cref{rjbound}, we have that with probability $1 - \delta/2$, 
\[
  \max_j \left|\langle \bX^j , \cE^Y\rangle\right| \leq
  \left(\max_{i\colon w_i \neq 0} |\cE^Y_i|\right) O\left(
    \sqrt{\frac{s}{n}}\ln(p/\delta)\right)
\]
\end{proof}
\fi

\paragraph{Wrapping up.} 
\iffalse
Recall that from our Kernel shrinkage result in \Cref{kernel-bound},
we have
$\Ex{}{\sup\{\|x- x_i\|\colon K(x, x_i, J) > 0 \}} =
O(s^{-\frac{1}{4\alpha d}})$, with
$\alpha = \frac{\log(\omega^{-1})}{\pi\log((1 - \omega)^{-1}) }$.
\swcomment{todo: plug in that bound}
\fi

We now have all the ingredients to apply \Cref{lasso-err}.

\begin{theorem}
  \iffalse Suppose that we set
  $s = \left( \frac{n k^2}{ \ln(p/\delta)} \right)^{\frac{2\alpha
      d}{2\alpha d+ 1}}$.\fi 

  Suppose that the tree learner satisfies the following shrinkage
  condtion
  \[
    \Ex{D_1, S^1, S^2}{\max_{i\in D_1}\|x - x_i\|_2\mid K(x_i, x,
      (S^1, S^2)) > 0} \leq O(s^{-\tau})
  \]
  Then with probability at least $1 - \delta$, the Lasso solutions
  $\hat q$ and $\hat \gamma$ satisfy
  \begin{align*}
    \|\hat q - q_0(x)\|_1 & \leq O\left(\frac{{k}}{\lambda_0} \left( \sqrt{\frac{s}{n}\ln(p/\delta)} + k s^{-\tau} \right)\right)\\
    \|\hat \gamma -\gamma_0 \|_1 & \leq O\left(\frac{{k}}{\lambda_0} \sqrt{\frac{s}{n} \ln(p/\delta)} \right)
  \end{align*}
  % \[
  %   \|\hat q - q_0(x)\|_2 \leq O\left(\sqrt{k}\left( k^{\frac{2\alpha
  %           d}{2\alpha d + 1}} \left(\frac{\ln(p/\delta)}{n}
  %       \right)^{\frac{1}{4\alpha d + 2}}\right) \right) = O\left(
  %     \frac{ k^{(6\alpha d + 1)}
  %       \ln(p/\delta)}{n}\right)^{\frac{1}{4\alpha d + 2}}
  % \]
  as long as the regularization parameter satisfies
  $\lambda_q \geq \Omega\left(\sqrt{\frac{s}{n}\ln(p/\delta)} + k
    s^{-\tau} \right)$,
  $\lambda_\gamma \geq
  \Omega\left(\sqrt{\frac{s}{n}\ln(p/\delta)}\right)$, and the sample
  size satisfies
  % \[
  %   n \geq \Omega(k^{2 + 8\alpha d} \left(\ln(p/\delta)\right)^{2 +
  %     2\alpha d})
  % \]
  \[
    n \geq \Omega(k^2 s \ln(p/\delta)).
  \]
\end{theorem}


\iffalse
\begin{proof}

  Using \Cref{rho-bound} for the restricted eigenvalue condition and
  \Cref{noise-bound}, we know from \Cref{lasso-thm} that with
  probability at least $1 - \delta$, 
  \[
    \|\hat q - q_0(x)\|_2 \leq O\left( \frac{\sqrt{k}}{\lambda_0 - O(k
        \sqrt{\frac{s}{n}\ln(p/\delta)})}
      \left(\sqrt{\frac{s}{n}\ln(p/\delta)} + k s^{-\frac{1}{4\alpha
            d}} \right)\right)
  \]
  \sw{need to say which version of lasso we use}

  Note that as long as
  \[
    n \geq \Omega(k^{2 + 8\alpha d} \left(\ln(p/\delta)\right)^{2 +
      2\alpha d})
  \]
  we will have
  $n \geq \Omega\left(\frac{k^2 s
      (\ln(p/\delta))^2}{\lambda_0^2}\right)$, we have
  \[
    \frac{1}{\lambda_0 - O\left(k \sqrt{\frac{s}{n}\ln(p/\delta)}
      \right)} \leq O(1)
  \]
  Then we can simplify the bound as
  \[
    \|\hat q - q_0(x)\|_2 \leq O\left( {\sqrt{k}}
      \left(\sqrt{\frac{s}{n}\ln(p/\delta)} + k s^{-\frac{1}{4\alpha
            d}} \right)\right)
  \]
  Moreover, if we set
  \[
    s = \left( \frac{n k^2}{ \ln(p/\delta)} \right)^{\frac{1}{1+
        \frac{1}{2\alpha d}}}
  \]
  then we can then rewrite
  \[
    \left(\sqrt{\frac{s}{n}\ln(p/\delta)} + k s^{-\frac{1}{4\alpha d}}
    \right) = O\left(k
      \left(\frac{\ln(p/\delta)}{nk^2}\right)^{\frac{1}{4 \alpha d +
          2}} \right) = O\left( k^{\frac{2\alpha d}{2\alpha d + 1}}
      \left(\frac{\ln(p/\delta)}{n} \right)^{\frac{1}{4\alpha d +
          2}}\right)
  \]
  This further simplifies the bound as
  \[
    \|\hat q - q_0(x)\|_2 \leq O\left(\sqrt{k}\left( k^{\frac{2\alpha
            d}{2\alpha d + 1}} \left(\frac{\ln(p/\delta)}{n}
        \right)^{\frac{1}{4\alpha d + 2}}\right) \right) = O\left(
      \frac{ k^{(6\alpha d +
          1)}  \ln(p/\delta)}{n}\right)^{\frac{1}{4\alpha d + 2}}
  \]
  which completes the proof.

\end{proof}


In other words, we obtain an error that is dinimising as sample size
grows as long as the sparsity parameter satisifes
\[
  k \leq O\left(\left(\frac{n}{(\ln(p/\delta))^{2 + 2\alpha
          d}}\right)^{\frac{1}{2 + 8\alpha d}} \right)
\]

\fi



\iffalse
\begin{lemma}[Follows from Theorem 11.1 of~\cite{{Lasso-Book}}]\label{awesome}
  Let $m = |L_b^2(x)|$.  Suppose that the design matrix of controls
  $\bX$ in the data set $L_b^2(x)$ has minimum eigenvalue at least
  $v$. Then as long as the Lasso regularization parameters satisfy
  $\lambda_\gamma \geq 2\|\bX^\intercal \cE^T\|_\infty/m$ and
  $\lambda_q \geq 2\|\bX^\intercal \cE^q\|_\infty/m$, the estimates
  $\hat \gamma_b$ and $\hat q_b$ satisfy
  \[
    \|\hat \gamma_b - \gamma_0(x) \| \leq \frac{3}{v}
    \sqrt{k}\lambda_\gamma,\quad \|\hat q_b - q_0(x) \| \leq
    \frac{3}{v} \sqrt{k}\lambda_q,
  \]
\end{lemma}

Note that for each of the noise vectors $\cE$ and any column $\bX_j$
of the matrix, we know that the random variable $\frac{1}{m}\bX_j \cE$
is a zero-mean Gaussian with variance at most
$O(\|\cE\|_\infty/m)$. Then the following $\ell_2$ error bound follows
immediately from \Cref{awesome} and the kernel shrinkage bound in
\Cref{kernel-bound}.

\begin{corollary}
  Let $m = |L_b^2|$. Then under \Cref{tree-ass} and \Cref{plrass},
  with probability at least $1 - \delta$, the following bounds hold as
  long as $p\leq \poly(n)$,
  \begin{align*}
    \|\gamma_0(x) - \hat \gamma_b\|_2,     \|q_0(x) - \hat q_b\|_2 \leq O\left(\sqrt{\frac{k\log(p)\log(n/\delta)}{m}} \right)
  \end{align*}
\end{corollary}
\fi
\fi

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "arxiv"
%%% End:


==> old_korf.tex <==
% !TEX root = nips_2018.tex
\section{Orthogonal Random Forest}
\label{sec:plr}
Now we describe our main algorithm \emph{orthogonal random forest}
(ORF) for the two stage estimation estimation. At a high level, ORF
can be viewed as an orthogonalized version of GRF that is more robust
to the nuisance estimation error. We will defer the details of the
first-stage nuisance estimation to \Cref{sec:kernel-lasso} and focus
on the second stage target estimation here. Similar to GRF, the
algorithm runs a tree learner over $B$ random subsamples $S_b$
(without replacement) to build $B$ trees such that each tree indexed
by $b$ provides a tree-based weight $a_{ib}$ for each observation
$Z_i$ in the input sample. Then we compute ORF weights over the
examples by averaging over the tree-weights, and solve for the ORF
estimator given by \Cref{weighted_moment}. 

The tree learner starts with a root node that contains the entire
$\cX$ and recursively grow the tree to split $\cX$ into a set of
leaves until the number of observations in each leaf is not too small.
The set of neighboods defined by the leaves naturally gives a
simlarity measure between each observation and the target $x$.
Following the same approach of \cite{GRF,WA}, we maintain the
following tree properties in the process of building a tree.
\begin{specification}[Forest Regularity]\label{forest_spec}
The tree construction process satisfies
\begin{itemize}
\item \textit{Honesty}: we randomly partition the input sample $S$
  into two subsets $S^1$, $S^2$, then uses $S^1$ to place splits in
  the tree, and uses $S^2$ for estimation.
\item $\omega$-\emph{balanced}: each split leaves at least a fraction
  $\omega$ of the observations in $S^2$ on each side of the split for
  some parameter of $\omega\leq 0.2$.
\item \textit{Minimum leaf size $r$}: there are between $r$ and
  $2r - 1$ observations from $S^2$ in each leaf of the tree. 
\item $\pi$-\emph{random-split}: at every step, marginalizing over the
  internal randomness of the learner, the probability that the next
  split occurs along the $j$-th feature is bounded below by $\pi/d$
  for some $0 < \pi \leq 1$, for all $j = 1, ..., d$ (e.g., this can
  be achieved by uniformly randomizing the splitting variable with
  probability $\pi$).
\end{itemize}
\end{specification}

The key modification to GRF's tree learner is our incorporation of
double ML in the splitting criterion. In order to accurately capture
the heterogeneity in the target parameter $\theta$ in the presence of
high-dimensional nuisance, we also perform a two-stage estimation at
each internal node to decide the next split. While the splitting
criterion does not factor into our theoretical analysis (similar to
\cite{GRF}), we find it to be an effective practical heuristic.

\paragraph{Splitting criterion with orthogonalization.}
At each internal node $P$ we perform a two-stage estimation over
$(P\cap S^1)$, i.e.~the set of examples in $S^1$ that reach node $P$:
1) first compute a nuisance estimate $\hat h_P$ given by the parameter
$\hat \nu_P$ that minimizes $\sum_{i\in (P\cap S^1)} \ell(Z_i; \nu)$,
and then 2) form estimate $\hat \theta_P$ using $\hat h_P$:
\[
  \hat \theta_P \in\argmin_{\theta\in \Theta} \left\|\sum_{i\in (P\cap
      S^1)} \psi(Z_i; \theta, \hat h_P(W_i)) \right\|
\]
Given the estimates $(\hat \theta_P, \hat h_P)$, we would like to find
an axis-aligned split of some node into two children $C_1$ and $C_2$
such that if we perform the same two-stage estimation separately at
each child, the new estimates $\hat \theta_{C_1}$ and
$\hat \theta_{C_2}$ take on very different values, so that the
heterogeneity of the two children nodes is maximized. However,
performing the two-stage estimation of $\hat \theta_{C_1}$ and
$\hat \theta_{C_2}$ for all possible splits is too computationally
expensive. Instead, we will approximate these estimates by taking a
Newton step from the parent node estimate $\hat \theta_P$: for any
child node $C$ given by a candidate split, our proxy estimate is then
given by
\[
  \tilde \theta_{C} = \hat \theta_P - \frac{1}{|C\cap S^1|}\sum_{i\in
    C} A_P^{-1} \psi(Z_i; \hat \theta_P, \hat h_P(W_i))
\] 
where
$A_P = \frac{1}{|P\cap S^1|} \sum_{i\in P\cap S_b^1} \nabla_\theta
\psi(Z_i; \hat \theta_P, \hat h_P(W_i))$.

Given the estimates $\tilde \theta_{C}$, we select the candidate split
that maximizes the following proxy heterogeneity score for the:
\begin{equation}\label{splitting}
  \tilde \Delta(C_1, C_2) = \sum_{j=1}^2 \frac{1}{|C_j\cap S^1|} \left(\tilde
    \theta_{C_j} -\hat \theta_P \right)^2
\end{equation}




\paragraph{ORF weights and estimator.}
For each tree indexed $b\in [B]$ based on subsample $S_b$, let
$L_b(x)\subseteq \cX$ be its leaf containing the target feature $x$,
and we assign \emph{tree weigh} and ORF weight to each observation
$i$:
\begin{align*}
  a_{ib} = \frac{\mathbf{1}[(x_i\in L_b(x)) \wedge (Z_i\in S_b^2)]}{|L_b(x) \cap S_b^2|}, \quad a_i = \frac{1}{B}\sum_{b=1}^B a_{ib}
\end{align*}
The ORF estimator $\hat \theta$ is then computed by solving the
weighted moment condition in \Cref{weighted_moment}.

\citet{WA} show that under the structural specification of the trees,
the tree weights are non-zero only around a small neighborhood of $x$.

\begin{theorem}[Kernel shrinkage \cite{WA}]\label{kernel-bound}
  Let $s$ be the subsample size. Suppose the minimum leaf size
  parameter $r = O(1)$ and tree is $\omega$-balanced and
  $\pi$-random-split. Further, assume that each feature $x_i$ is drawn
  independently from the uniform distribution over $[0, 1]^d$. Then
  the tree weights satisfies
  $\Ex{}{\sup\{\|x- x_i\|\colon a_{ib} > 0 \}} =
  O(s^{-\frac{1}{2\alpha d}})$, with
  $\alpha = \frac{\log(\omega^{-1})}{\pi\log((1 - \omega)^{-1}) }$.
\end{theorem}

\iffalse
\begin{algorithm}[h]
\begin{algorithmic}[1]
  \STATE{\textbf{Input}: a dataset $D$ of size $n$, target point $x$,
    kernel base learner $\cL_k$, parameter $B$: number of kernels,
    parameter $s$ subsample size} 

  \STATE{Randomly split the data set $D$ into two data sets of equal
    size $D_1$ and $D_2$}
  \STATE{\textbf{First stage: nuisance estimation.}}
  \STATE{Compute nuisance estimate $\hat h$ by performing a kernel
    nuisance estimation using dataset $D_1$}

    \STATE{\textbf{Second stage: moment estimation with $\hat h$}.}

    \STATE{For each $Z_i\in D_2$, set weight $a_{ib} = 0$ for all
      $b\in[B]$}

    \STATE{\textbf{For} $b = 1 ,\ldots , B$: }

    \INDSTATE{Let $S_{b}$ be a set of $s$ observations randomly
      subsampled without replacement from $D_2$}
    % ; Randomly partition
    % $S_{b}$ into two data sets of even size: $S_{b}^1$ and
    % $S_{b}^2$

    \INDSTATE{Run tree learner on $S_b$ and compute tree weight on
      each observation $i\in D_2$.}
    \STATE{\textbf{For} each $Z_i\in D_2$, let $a_i = \frac{1}{B}\sum_{b=1}^B a_{ib}$}
  \STATE{Compute $\hat \theta$ by solving the weighted moment
    condition in \Cref{weighted_moment}.
    }
    \caption{Orthogonal Random Forest}
  \label{alg:mainalg}
\end{algorithmic}
\end{algorithm}
\fi

We will leverage this kernel shrinkage result in our analysis.

\section{Convergence and Asymptotic Analysis}\label{sec:conv-rate}
\iffalse
\paragraph{Base kernel learner.} The learner $\cL_k$ takes a set $S$
of observations as input, and outputs a kernel weighting function
$K\colon \cX\times \cX \times \cZ^m \rightarrow [0,1]$. In particular,
given any target feature $x$ and a set of observations $S$, the weight
of each observation $Z_i$ in $S$ with feature vector $x_i$ is
$K(x_i, x, S)$. For the convenience of our analysis, we will assume
that the weights among the observations in $S$ are non-negative and
normalized such that $\sum_{Z_i \in S} K(x_i, x, S) = 1$.


% Following the approach of generalized random forest (GRF) by
% \citet{ATW17}, we estimate $\theta_0(x)$ by first assigning a set of
% similarity weights over the observations, and then computing
% $\hat \theta$ via a kernel regression with the set of
% weights. However, to overcome the confounding effects from the
% high-dimensional controls $W_i$, we rely on double ML method due
% to~\cite{doubleML} that orthogonalizes the effects from $W_i$ when
% estimating $\theta$. We will first introduce our forest-based kernel
% learner, and then describe how orthogonal random forest (ORF) uses
% it to perform kernel estimation.

Following the approach of generalized random forest (GRF) by
\citet{ATW17}, we run the base kernel learner on $B$ random subsamples
and take the average over the kernel weights to obtain the similarity
weights $a_i$. This allows us to analyze the weighted score as a
$U$-statistic, which is important for establishing convergence rate
and asymptotic normality.

The formal description of estimation procedure in \Cref{alg:mainalg}.
To analyze our estimator, we rely on several assumptions on the moment
condition and the kernel learner.
\fi

To provide theoretical guarantees for ORF, we reluy on the following
assumption on the local moment conditions.
\begin{assumpt}\label{tech-conditions}
  The moment condition and the score function satisfy the following:
\begin{enumerate}
\item \textbf{Local Orthogonality.} The moment condition satisfies
  local orthogonality.
\item \textbf{Identifiability.}  The moments $m(x; \theta, h_0)=0$ has
  a unique solution $\theta_0(x)$.
% , i.e.
  % $\forall \epsilon > 0: \inf\{ \|m(x; \theta, h_0)\|: \|\theta -
  % \theta_0(x)\| \geq \epsilon\} > 0$

\item \textbf{Curvature.} The Jacobian
  $\nabla_\theta m(x; \theta_0(x), h_0)$ has minimum eigenvalue
  bounded away from zero.
\item \textbf{Smoothness of moments.} For every $j\in [p]$ and for all
  $\theta$ and $h$, the eigenvalues of the expected Hessian
  $\Ex{}{\nabla^2_{(\theta, h)} \psi_j(Z; \theta, h(W))\mid x, W}$ \vscomment{I think we also need to condition on $W$ for the proof, which I added. We might as well assume it point-wise for simplicity.} are
  bounded above by a constant $O(1)$.  For any $Z$, the score
  $\psi(Z; \hat \theta, \hat \nu)$ is $O(1)$-Lipschitz in
  $\hat \theta$ for any $\hat \nu$ and $O(1)$-Lipschitz in $\hat \nu$
  for any $\hat \theta$.

\item \textbf{Boundedness.} The parameter set $\Theta$ has constant
  diameter.  There exists a bound $\psimax$ such that for any
  observation $Z$, the first-stage nuisance estimate $\hat h$
  satisfies {$\|\psi(Z; \theta, \hat h)\|_{\infty}\leq \psimax$} for
  any $\theta\in \Theta$.

% \item The subsampling parameter is chosen such that
%   $s^{-\tau} + \psimax \sqrt{s\ln(n)/n} = o(1)$.

\end{enumerate}
\end{assumpt}

Note that except for the local orthogality condition, all of the
assumptions are imposing standard boundedness and regularity
conditions of the moments.



\iffalse
Next, we will turn to our assumptions on the kernel learner.
\begin{assumpt}[Assumption Kernel Learner]\label{shrinkage}
  The learner takes as input a set $S$ consisting of $s$
  i.i.d. observations drawn from $\cD$ and satisfies the following:
\begin{enumerate}
\item \textit{Kernel Shrikage.} The kernel weights satisfy
\begin{equation*}
  \Ex{}{\sup \left\{\|x - x_i\|_2: K(x_i, x, S) > 0 \right\}} = O\left(s^{-\tau}\right)
\end{equation*}
\item \textit{Honesty.} For any observation $i$, the weight
  $K(x_i, x, S)$ is independent of $Z_i$, conditioned on realized
  feature being $x_i$.
\end{enumerate}
\end{assumpt}

The first assumption asserts that the weights are \emph{localized}
around the target $x$. The second assumption ensures that the
high-dimensional nuisance of the observation does not influence the
weight calculatino. We will establish both of these conditions for our
variant of generalized random forest.\swcomment{pls check}
\fi



% Our GMM estimation algorithm can be viewed as a genearlization of
% ORF. It divides the input dataset $D$ into two disjoint subsets $D_1$
% and $D_2$, uses a kernel learner to assign importance weights $a_i$
% over the observations in the two sets. Then it performs a similar
% two-stage estimation: first compute a nuisance estimate $\hat h$ via a
% kernel estimation on $D_2$, and then compute the final estimate
% $\hat \theta$ by solving weighted moment condition over $D_2$:
% $\sum_{Z_i\in D_2} a_{i} \psi(Z_i; \hat\theta, \hat h(W_i)) = 0$.  




\iffalse
In the second stage, we use techniques from orthogonal machine
learning to compute the estimate $\hat \theta$ by solving the weighted
moment condition. The formal procedure is described in
\Cref{alg:stage-two}.

\begin{algorithm}[htpb]
  \label{alg:stage-two}
\begin{algorithmic}
  \STATE{\textbf{Input}: data set $S$, target point $x$, Kernel
    function $\hat{K}(x, x_i, S)$ using an auxiliary sample $S'$, such
    that $\sum_{i=1}^n \hat{K}(x, x_i, S)=1$. }


 \STATE Using a samples $S''$
  estimate nuisance function $\hat{h}$ \STATE For each data target
  $x$, estimate $\theta(x)$ by solving the local empirical moment:
\begin{equation}
\sum_{i\in S} \hat{K}(x, x_i, S_{-i})\cdot \psi(Z_i; \theta, \hat{h})=0
\end{equation}
\end{algorithmic}
\caption{Stage 2: estimation via orthogonal machine learning}
\label{alg:general}
\end{algorithm}

We make the following assumptions on the estimated kernels:
\begin{assumpt}[Kernel Averaging and Honesty] The estimated Kernel is
  an average over $B$ Kernels created based on sub-sampled data sets:
\begin{equation}
K(x_i, x, S_{-i}) = \frac{1}{B} \sum_{b=1}^B K_b(x_i, x, S_{-i})
\end{equation}
and $K_b(\cdot, \cdot, \cdot)$ is estimated on a sub-sample without replacement of size
$s$ of an auxiliary independent dataset $S'$ of size $n$.
\end{assumpt}
\fi


\vsedit{Now we state the convergence guarantee of
  $\|\hat \theta - \theta_0(x)\|$.}




\begin{theorem}\label{thm:converge}
  Suppose that the marginal each feature vectors $x_i$ are
  independently and uniformly distributed over $[0, 1]^d$ and that the
  moment conditions satisfy \Cref{tech-conditions}. {If the first stage
  estimates are consistent at a sufficiently fast rate:
\begin{align*}
  &\Ex{}{\|\hat h(W) - h_0(W)\|^2\mid x}\\ \leq &{o}_p\left(\left( s^{-\tau} +
    \psimax\sqrt{\frac{s \, p\, \ln(p\, n/ s)}{n}} \right) \right)
  \end{align*}
and the second stage estimate is consistent, i.e. $\Ex{}{ \|\hat{\theta} - \theta_0(x)\|} = o_p(1)$, 
then the first stage estimation error can asymptotically be ignored and the final stage estimate $\hat{\theta}$ converges at an oracle rate of:
\begin{align*}
&\Ex{}{ \|\hat
    \theta - \theta_0(x) \|} \\\leq &{O}\left( \sqrt{p} \left(s^{-\tau} +
    \psimax\sqrt{\frac{s \, p\, \ln(p\, n/ s)}{n}} \right) \right)
\end{align*}}
\end{theorem}

\swcomment{add a remark here.}  

In this section, we will assume consistency of the overall estimation
process, i.e. that $\|\hat \theta - \theta_0(x)\| = o_p(1)$, and prove
a rate of convergence conditional on consistency. In the next section
we will also argue consistency under some extra set of convexity
conditions. In essence, consistency allows us to restrict the estimate
$\hat{\theta}$ in a cone around the true parameter, such that
$\|\hat{\theta}-\theta_0(x)\|^2 < \kappa_n
\|\hat{\theta}-\theta_0(x)\|$, for some $\kappa_n = o_p(1)$. Within
this cone, we prove an explicit convergence rate of the estimation
error.  We have a stronger consistency rate when the score is a
gradient of loss.



\iffull First, we will bound the estimation error as a sum of
$m(x; \theta, \hat h)$ and second order terms. The proof follows from
the Taylor expansion of the moment function and mean-value theorem
(see appendix).


\begin{lemma}\label{lem:taylor}
  Under \Cref{tech-conditions}, for any nuisance estimate $\hat h$ and
  parameter $\theta$,
  \begin{align*}
   & \|\theta - \theta_0(x)\| \leq \mathcal{O} \left( \left\|m(x; \theta, \hat h)\right\| \right)\\ + &\sqrt{p}\, \mathcal{O}\left(\Ex{}{\|\hat h(W) - h_0(W)\|^2\mid x}
      +\|{\theta}-\theta_0(x)\|^2\right).
  \end{align*}
\end{lemma}





Next, we will fix the nuisance estimate $\hat h$ and define the
following functions of $\theta$:
\begin{align*}
  \Psi(\theta) &= \sum_{i: Z_i \in D_2} a_{i} \, \psi(z_i;
                 \theta, \hat h(W_i)), \\
  \Lambda_n(\theta) &=   m(x; {\theta}, \hat{h}) - \Psi(\theta)
%  =  \frac{1}{B}\sum_{b=1}^B m(x; {\theta}, \hat{h}_b) - \frac{1}{B}\sum_{b=1}^B  \sum_{i=1}^n a_{ib} \cdot \psi(z_i;
                      % {\theta}, \hat{h}_b)
%  =\frac{1}{B}
                % \Ex{}{\sum_{b=1}^B \sum_{i=1}^n a_i \psi(z_i; \theta, \hat h_b)}
\end{align*}



% Recall that the true parameter $\theta_0 = \theta(x)$ is the solution
% to the equation:
% \begin{equation}\label{eqn:true-moment}
% % \Ex{}{\psi(z; \theta_0, h_0) | x} 
% m(x; \theta_0, h_0)= 0
% \end{equation}
% and
Recall that our estimate $\hat{\theta}$ at the target point $x$ is the
solution to the equation: $\Psi(\hat{\theta}, \hat{h}) =
0$. Equivalently, we can also view $\hat \theta$ as the solution for
$m(x; \hat\theta , \hat h)= \Lambda_n(\hat \theta)$.  This means we
can decompose the error as
\begin{align*}
&  \|\hat \theta - \theta_0(x)\| = O\left(\left\|\Lambda_n(\hat \theta )
    \right\| \right)\\ +  &O\left(\sqrt{p}\, \left(\Ex{}{\|\hat h(W) -
      h_0(W)\|^2\mid x} +\|\hat{\theta}-\theta_0(x)\|^2\right) \right)
\end{align*}

Note that under our assumption on the first stage estimation error
rate and condition that the second stage estimator is consistent, both
of the second-order terms $\Ex{}{\|\hat h(W) - h_0(W)\|^2\mid x}$ and
$\|\hat{\theta}-\theta_0(x)\|^2$ will be in smaller order than
$\|\hat \theta - \theta_0(x)\|$. We will defer the proof of
consistency to the appendix and focus on bounding the scale of
${\Lambda_n(\theta)}$ for any $\theta\in \Theta$.


\vsedit{\begin{lemma}[Uniformly Bounding
    $\Lambda_n(\theta)$]\label{lem:lambda-n} For any $x$:
\begin{equation}
\Ex{}{\sup_{\theta \in \Theta} \|\Lambda_n(\theta)\|_{\infty}} = {O}\left( s^{-\tau} +
    \psimax\sqrt{\frac{s\ln(n)}{n}}\right) 
\end{equation}
\end{lemma}}

\begin{proof}[Proof sketch of \Cref{lem:lambda-n}]
  We will rewrite the expression of $\Lambda_n(\theta)$ by adding and
  subtracting the term $\mu(\theta) = \Ex{}{\Psi(\theta)}$, where the
  expectation is taken over both the random draws of the observations
  and the internal randomness of the algorithm. By leveraging the
  honesty property of the kernel weights, we can rewrite $\mu(\theta)$
  as the following.
\begin{lemma}\label{exp-proof}
  For any $\theta$,
  $$\mu(\theta) = \Ex{}{\sum_{i: Z_i \in D_2} a_{i}\,
    m(x_i; \theta,\hat h)}.$$
\end{lemma}


Then we can decompose $\Lambda_n(\theta)$ as a sum of two error terms
such that the first one is \emph{kernel error} due to the kernel
averaging around a neighborhood of $x$, and the second one is
\emph{sampling error} due to the sampling error of the moment:
\begin{align*}
  &\Lambda_n(\theta)  =~  m(x; {\theta}, \hat{h}) - \mu({\theta}) +  \mu({\theta}) - \Psi(\theta)\\
  &  = \underbrace{\Ex{}{\sum_{i: Z_i \in D_2} a_{i}\cdot \left(m(x; {\theta}, \hat{h}) - m(x_i; {\theta}, \hat{h})\right)}}_{\Gamma(\theta)=\text{kernel error}}
    \\ & + \underbrace{\mu(\theta) - \frac{1}{B} \sum_{b=1}^B \sum_{i:Z_i \in D_2} a_{ib} \cdot \psi(Z_i; {\theta}, \hat{h})}_{\Delta(\theta)=\text{sampling error}}
\end{align*}

By the assumption of kernel shrinkage and the Lipschitzness of the $m$
in the first input $x$, we can bound the kernel error by
$O(s^{-\tau})$. To bound the sampling error, first observe that
$\sum_{i: Z_i\in D_2} a_{ib}\cdot \psi_j(Z_i; {\theta}, \hat{h})$ is
computed based on a random sub-sample of $D_2$ (without replacement),
and thus each coordinate $\Psi_j(\theta)$ can be viewed as a Monte
Carlo approximation to a $U$-statistic, centered at
$\mu_j(\theta)$. Hence, we can bound the sampling error with high
probability using concentration inequality. Finally, to uniformly
bound the sampling error for all $\theta$, we will apply union bound
over an $\eps$-cover over the set $\Theta$, for sufficiently small
value of $\eps$.
\end{proof}


\begin{proof}[proof of \Cref{thm:converge}]
  By \Cref{lem:lambda-n}, we have
  $\Lambda_n(\hat \theta) \leq \sqrt{p} \, {O}\left( s^{-\tau} +
    \psimax\sqrt{\frac{s \, p\, \ln(p\, n/ s)}{n}}\right) \equiv E$.
  Since $\hat \theta$ is consistent (proof deferred in the appendix),
  the second term $\|\hat\theta - \theta_0(x)\|^2$ is at most
  $\frac{1}{2}\|\hat{\theta} - \theta_0(x)\|$. Further, since the
  nuisance estimation error term is in smaller order than
  $E/\sqrt{p}$, we can bound $\|\hat{\theta} - \theta_0(x)\| \leq E$,
  as desired.
\end{proof}



%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main.tex"
%%% End:


==> sketch.tex <==
\paragraph{Proof Sketch of~\Cref{thm:final-hetero-te}}
% \label{sec:sketch}

To prove the convergence rate of ORF using \Cref{thm:converge}, we
need two technical ingredients. The first one is to establish the
kernel shrinkage condition for tree learner---that is the rectangle
defined at each leaf is shrinking at a certain rate as the subsample
size $s$ grows. The following result follows from Lemma 2
of~\cite{WA}.


\begin{lemma}[Kernel shrinkage of a tree learner]\label{kernel-bound}
  Suppose for any input data set of size $s$, the minimum leaf size
  parameter of the tree learner is set to be $r = O(1)$. Then under
  Assumptions \ref{tree-ass} and \ref{plrass} and that the dimension
  $d = O(1)$. Then the kernel weighting function output by the tree
  learner satisfies
  $\Ex{}{\sup\{\|x- x_i\|\colon K(x, x_i, S) > 0 \}} = O(s^{-\tau})$,
  with $\tau = \frac{1}{2\alpha d}$ and
  $\alpha = \frac{\log(\omega^{-1})}{\pi\log((1 - \omega)^{-1}) }$.
\end{lemma}


The second ingredient is to establish the accuracy guarantee of the
kernel Lasso method as our nuisance estimation. In PLR, to bound the
error of the nuisance estimate $\hat h$, it suffices to bound the
$\ell_1$ errors $\|\hat q - q_0(x)\|_1$ and
$\|\hat \gamma -\gamma_0\|_1$. Our analysis deviates from the standard
Lasso analysis in that (1) the sparse vector $q_0(x_i)$ for each
feature $x_i$ is different, which introduces adversarial error and (2)
the tree learner will place non-uniform weights over the
observations. To address these issues, we bound the adversarial error
using the kernel shrinkage of the tree learner, and establish the
restricted eigenvalues condition of the weighted covariance matrix by
using concentration of U-statistics. 

\begin{theorem}[Kernel Lasso accuracy]\label{lasso-err}
  Suppose that the tree learner satisfies the kernel shrinkage
  condition with parameter $\tau$.  Then with probability at least
  $1 - \delta$, the Lasso solutions $\hat q$ and $\hat \gamma$ satisfy
  \begin{align*}
    \|\hat q - q_0(x)\|_1  \leq O\left(\frac{{k}}{\lambda_0} \left( \sqrt{\frac{s}{n}\ln(p/\delta)} + k s^{-\tau} \right)\right), \qquad
    \|\hat \gamma -\gamma_0 \|_1 \leq O\left(\frac{{k}}{\lambda_0} \sqrt{\frac{s}{n} \ln(p/\delta)} \right)
  \end{align*}
  as long as the regularization parameter satisfies
  $\lambda_q \geq \Omega\left(\sqrt{\frac{s}{n}\ln(p/\delta)} + k
    s^{-\tau} \right)$,
  $\lambda_\gamma \geq
  \Omega\left(\sqrt{\frac{s}{n}\ln(p/\delta)}\right)$, and the sample
  size satisfies $n \geq \Omega(k^2 s \ln(p/\delta))$.
\end{theorem}






%%% Local Variables:
%%% mode: latex
%%% TeX-master: "nips_2018"
%%% End:


==> wrap_up.tex <==
\section{Analysis of Orthogonal Random Forest}\label{simple-analysis}


Finally, we will use the tools we develop in the previous sections to
provide a full analysis for the ORF algorithm. We need to combine two
main technical ingredients to invoke our general convergence result of
\Cref{thm:converge}. First, we need to show the tree learner satisfy
the kernel shrinkage assumption. Second, we rely on the kernel Lasso
analysis in \Cref{sec:kernel-lasso} to bound the nuisance estimation
error.


\subsection{Kernel Shrinkage for Tree Learners}\label{sec:rf-learner-2}
The analysis on kernel
shrinkage rate essentially follows from the result of \cite{WA} on the
localization of the kernel weights.

\iffalse In particular, we will rely on the same set of assumptions
imposed in \cite{WA,ATW17}.

\begin{assumpt}[Tree learner assumption]\label{tree-ass}
  We assume the tree learner $\cL_T$ takes a data set $S$ as input,
  randomly partition $S$ as two random subsets $S^1, S^2$ of equal
  sizes, and builds a tree that is
\begin{itemize}
 \item $\omega$-\emph{regular} for $\omega\leq 0.2$: each split leaves
  at least a fraction $\omega$ of the observations in $S^2$ on each side
  of the split and, moreover, the trees are fully grown to depth $k$
  for some $k \in \NN$, i.e., there are between $r$ and $2r - 1$
  observations in each leaf of the tree.

\item \emph{a random-split tree}: if at every step of the tree-growing
  procedure, marginalizing over the internal randomness of the
  learner, the probability that the next split occurs along the $j$-th
  feature is bounded below by $\pi/d$ for some $0 < \pi \leq 1$, for
  all $j = 1, ..., d$.
\end{itemize}
\end{assumpt}
\fi
\begin{lemma}[Follows from Lemma 2 of~\cite{WA}]\label{detailed-shrinkage}
  Consider the tree learner as the base kernel learner $\cL_k$ under
  \Cref{tree-ass}. Then given a set of observations
  $S = (Z_1, \ldots , Z_s)$ such that the associated feature vectors
  $x_1, \ldots , x_s$ are drawn independently from uniform
  distribution $U([0, 1]^d)$. Let $L(x)$ be the leaf containing the
  target feature vector $x$. Then for sufficiently large enough $s$,
\[
  \Pr\left[ \textrm{diam}(L(x)) \geq \sqrt{d} \left( \frac{s}{2 r -
        1}\right)^{\frac{-0.51}{\alpha d}}\right] \leq d\left(
    \frac{s}{2r - 1}\right)^{\frac{-1}{2\alpha d}}
\]
where $r$ is the minimum number of points from $S^2$ that fall in each
leaf, $\textrm{diam}(L(x))$ denotes the diameter inside the leaf
$L(x)$ and
$\alpha = \frac{\log(\omega^{-1})}{\pi\log((1 - \omega)^{-1}) }$.
\end{lemma}


\begin{corollary}[Kernel shrinkage of a tree learner]\label{kernel-bound}
  Suppose for any input data set of size $s$, the minimum leaf size
  parameter of the tree learner is set to be $r = O(1)$. Then under
  \Cref{tree-ass} and assume that the dimension $d = O(1)$. Then the
  kernel weighting function output by the tree learner satisfies
  $\Ex{}{\sup\{\|x- x_i\|\colon K(x, x_i, S) > 0 \}} =
  O(s^{-\frac{1}{2\alpha d}})$, with
  $\alpha = \frac{\log(\omega^{-1})}{\pi\log((1 - \omega)^{-1}) }$.
\end{corollary}


\iffalse
\begin{lemma}\label{noise-bound}
  Under \Cref{tree-ass} and \Cref{plrass}, for any
  $\delta \in (0, 1)$, with probability at least $1 - \delta$, the
  following bound holds as long as $B\geq (n/s)$,
\[
  \|\bX^\intercal \tilde\cE^Y\|_\infty \leq
  O\left(\sqrt{\frac{s}{n}\ln(p/\delta)} + k\; s^{-\frac{1}{4\alpha
        d}} \right)
\]
with $\alpha = \frac{\log(\omega^{-1})}{\pi\log((1 - \omega)^{-1}) }$.
\end{lemma}

\subsection{Convergence Rate}
\fi

\subsection{Wrapping up: proof of \Cref{thm:final-hetero-te}.} 
By the kernel shrinkage result in \Cref{kernel-bound}, we have
\[
    \Ex{D_1, S^1, S^2}{\max_{i\in D_1}\|x - x_i\|_2\mid K(x_i, x,
      (S^1, S^2)) > 0} \leq O(s^{-\tau})
\]
with $\tau = \frac{1}{2\alpha d}$ and
$\alpha = \frac{\log(\omega^{-1})}{\pi\log((1 - \omega)^{-1}) }$.  By
\Cref{lasso-err}, we can bound the $\ell_1$ Lasso error: with
probability at least $1 - \delta$,
\begin{align*}
{\|\hat q - q_0(x)\|_1}  \leq O\left(\frac{{k}}{\lambda_0} \left( \sqrt{\frac{s}{n}\ln(p/\delta)} + k s^{-\tau} \right)\right),\qquad
{ \|\hat \gamma -\gamma_0 \|_1} \leq O\left(\frac{{k}}{\lambda_0} \sqrt{\frac{s}{n} \ln(p/\delta)} \right)
\end{align*}
Recall that the error of the nuisance estimate $\hat h$ can be written
as
\begin{equation}\label{lasso-acc}
  \|\hat h(W) - h_0(W)\|_2^2 = (\langle \hat q - q_0(x), W\rangle)^2 +
  (\langle \hat \gamma - \gamma_0, W\rangle)^2
\end{equation}
In the remainder of the proof, we set $\delta = 1/n$ and define the
Lasso condition in \Cref{lasso-acc} as event $E$. By H\"{o}lder
inequality, we can also bound,
\[
  \Ex{}{ \|\hat h(W) - h_0(W)\|_2^2 \mid x, E} \leq
  O\left(\frac{{k}}{\lambda_0} \left( \sqrt{\frac{s}{n}\ln(p)} + k
      s^{-\tau} \right)\right)
\]


By \Cref{lem:psimax}, we know that under the event $E$ that
$\psimax\leq O(k)$ as long as
$\|\hat q - q_0(x)\|, \|\hat \gamma - \gamma_0\|\leq O(1)$. Then by
\Cref{thm:converge}, we know 
\[\mbox{ if }
  \Ex{}{\|\hat h(W) - h_0(W)\|^2\mid x, E} \leq {O}\left( s^{-\tau} +
    k\sqrt{\frac{s\ln(n)}{n}}\right) \mbox{ then } \Ex{}{ |\hat
    \theta - \theta_0(x)|\mid E} \leq {O}\left( s^{-\tau} +
    k\sqrt{\frac{s\ln(n)}{n}}\right)
  \]
  Note that if we set
  $s =\left(\frac{n}{k^2\ln(p)} \right)^{\frac{1}{1 + 2\tau}}$, then
  $s^{-\tau} = k\sqrt{\frac{s\ln(p)}{n}}$ and
  $$s^{-\tau} + k\sqrt{\frac{s\ln(n)}{n}} =
  \Theta\left(\left(\frac{n}{k^2\ln(p)}\right)^{\frac{-\tau}{1 +
        2\tau}}\right)$$ 
Furthermore, if the support size satisfies
  $k\leq \left(\frac{n}{\ln(p)}\right)^{\frac{\tau}{10\tau + 4}}$,
  then
  \[
    \Ex{}{\|\hat h(W) - h_0(W)\|^2\mid x, E} \leq
    O\left(\left(\frac{n}{k^2\ln(p)}\right)^{\frac{-\tau}{1 +
          2\tau}}\right)
\]
This implies that 
  \[
    \Ex{}{| \hat \theta - \theta_0(x) |\mid E} \leq
    O\left(\left(\frac{n}{k^2\ln(p)}\right)^{\frac{-\tau}{1 +
          2\tau}}\right)
\]
Finally, since the range of $\hat \theta$ is bounded, we know that
$\Ex{}{|\hat \theta - \theta_0(x)| \neg E} = O(1/n)$, which has lower
order than $\Ex{}{| \hat \theta - \theta_0(x) |\mid E}$. This recovers
our final stated bound.  \iffalse
\begin{theorem}\label{thm:final-hetero-te}
  Under \Cref{tree-ass} and \Cref{plrass}, the output estimate
  $\hat \theta$ by the kernel orthogonal random forest satisfies
\[
  \Ex{}{|\hat \theta - \theta_0(x)|} \leq O\left( \left(\frac{\ln
        p}{n} \right)^{\frac{\tau}{{2\tau + 1}}} \right)
\]
as long as the sparsity of the linear functions $\beta_0$ and
$\gamma_0$ satisfy 
\[
  k \leq O\left(\left(\frac{n}{\ln p} \right)^{\frac{\tau}{6\tau + 3}}\right)
\]
and we set the subsample parameter to be
$$s = \left(\frac{n}{\ln{p}}\right)^{\frac{1}{2\tau + 1}}$$ where
$\tau = \frac{1}{2\alpha d}$ and
$\alpha = \frac{\log(\omega^{-1})}{\pi\log((1 - \omega)^{-1}) }$.
\end{theorem}
\fi








%%% Local Variables:
%%% mode: latex
%%% TeX-master: "nips_2018"
%%% End:

